Symbolic Snapshot Ensembles

Inductive logic programming (ILP) is a form of logical machine learning. Most ILP algorithms learn a single hypothesis from a single training run. Ensemble methods train an ILP algorithm multiple times to learn multiple hypotheses. In this paper, we train an ILP algorithm only once and save intermediate hypotheses. We then combine the hypotheses using a minimum description length weighting scheme. Our experiments on multiple benchmarks, including game playing and visual reasoning, show that our approach improves predictive accuracy by 4% with less than 1% computational overhead.

==> plot_three_scatter.tex <==
\begin{figure*}[ht!]
  \centering
  %── Load the one-column raw vectors ──────────────────────────────────
  \pgfplotstableread[col sep=space]{data_lines/diff_testopt_minus_ensemble_errorsize.txt}\dataTestErr
  \pgfplotstableread[col sep=space]{data_lines/diff_worst_minus_ensemble_errorsize.txt}\dataWorstErr
  \pgfplotstableread[col sep=space]{data_lines/diff_testopt_minus_ensemble_fnsize.txt}\dataTestFn
  \pgfplotstableread[col sep=space]{data_lines/diff_worst_minus_ensemble_fnsize.txt}\dataWorstFn
  \pgfplotstableread[col sep=space]{data_lines/diff_testopt_minus_ensemble_mdl.txt}\dataTestMdl
  \pgfplotstableread[col sep=space]{data_lines/diff_worst_minus_ensemble_mdl.txt}\dataWorstMdl

  %── Merge X (test-opt) and Y (worst) into the same table ─────────────
  \pgfplotstablecreatecol[
      copy column from table={\dataWorstErr}{[index]0}
  ]{Y}{\dataTestErr}

  \pgfplotstablecreatecol[
      copy column from table={\dataWorstFn}{[index]0}
  ]{Y}{\dataTestFn}

  \pgfplotstablecreatecol[
      copy column from table={\dataWorstMdl}{[index]0}
  ]{Y}{\dataTestMdl}

  %── Draw the three scatter sub-plots ─────────────────────────────────
  \begin{tikzpicture}
    \begin{groupplot}[
        group style={
          group size=3 by 1,
          horizontal sep=5.6em,
        },
        width=0.31\textwidth,
        height=0.23\textwidth,
        xlabel={$ACC_{\text{test-opt}}\!-\!ACC_{\text{ens}}$},
        ylabel={$ACC_{\text{worst}}\!-\!ACC_{\text{ens}}$},
        xmin=-0.4, xmax=0.1,
        ymin=-0.4, ymax=0.1,
        xmajorgrids, ymajorgrids,
        enlargelimits=true,
        scatter/only marks,
        scatter,
        mark=*,
        mark size=1.6pt
      ]

      %── (1) ErrorSize ────────────────────────────────────────────────
      \nextgroupplot[
        title={\textsc{ErrorSize}}
      ]
      \addplot table[x index=0, y=Y]{\dataTestErr};
      \addplot[dashed, gray] coordinates {(-1,-1) (1,1)};  % y = x reference

      %── (2) LexFnsize ───────────────────────────────────────────────
      \nextgroupplot[
        title={\textsc{LexFnsize}}
      ]
      \addplot table[x index=0, y=Y]{\dataTestFn};
      \addplot[dashed, gray] coordinates {(-1,-1) (1,1)};

      %── (3) MDL ─────────────────────────────────────────────────────
      \nextgroupplot[
        title={\textsc{MDL}}
      ]
      \addplot table[x index=0, y=Y]{\dataTestMdl};
      \addplot[dashed, gray] coordinates {(-1,-1) (1,1)};
    \end{groupplot}
  \end{tikzpicture}

  \caption{Per-task comparison of ensemble accuracy gaps under the three cost functions.}
  \label{fig:delta-ensemble-scatter}
\end{figure*}

